Revisiting Single Image Reflection Removal In the Wild

This research focuses on the issue of single-image reflection removal (SIRR) in real-world conditions, examining it from two angles: the collection pipeline of real reflection pairs and the perception of real reflection locations. We devise an advanced reflection collection pipeline that is highly adaptable to a wide range of real-world reflection scenarios and incurs reduced costs in collecting large-scale aligned reflection pairs. In the process, we develop a large-scale, high-quality reflection dataset named Reflection Removal in the Wild (RRW). RRW contains over 14,950 high-resolution real-world reflection pairs, a dataset forty-five times larger than its predecessors. Regarding perception of reflection locations, we identify that numerous virtual reflection objects visible in reflection images are not present in the corresponding ground-truth images. This observation, drawn from the aligned pairs, leads us to conceive the Maximum Reflection Filter (MaxRF). The MaxRF could accurately and explicitly characterize reflection locations from pairs of images. Building upon this, we design a reflection location-aware cascaded framework, specifically tailored for SIRR. Powered by these innovative techniques, our solution achieves superior performance than current leading methods across multiple real-world benchmarks. Codes and datasets will be publicly available.

==> Sec1_intro.tex <==
\section{Introduction}

% Photography in the presence of reflective materials (\eg, glasses) often unavoidably results in the occurrence of reflections. These underside reflections will significantly disrupt the aesthetic visual perception of captured images and degrade the accuracy of the subsequent computer vision applications~\cite{sinha2012image, liu2020reflection,qiu2023looking}. Hence, it is important and meaningful to develop effective reflection removal algorithms.

In photographic environments involving reflective materials, such as glass, the inadvertent emergence of reflections is a common challenge. These underside reflections not only diminish the aesthetic quality of the captured images but also impede the accuracy of follow-up computer vision tasks~\cite{sinha2012image, liu2020reflection,qiu2023looking}. Consequently,  devising effective reflection removal algorithms is important and meaningful.


% According to the physical reflection formulation~\cite{fan2017generic, yang2018seeing, zhang2018single}, the reflection image $\textbf{M}$ can be considered as the superimposed transmission layer $\textbf{T}$ and reflection layer $\textbf{R}$. Obviously, due to the fundamental ill-posedness of removing reflection disturbance, traditional approaches devise various pre-defined assumptions, \eg, handcrafted assistance~\cite{levin2007user, ahmed2021user}, multiple frames~\cite{guo2014robust,xue2015computational} ghosting effects~\cite{shih2015reflection}, and gradient 
% priors~\cite{wan2018region,sun2016automatic, arvanitopoulos2017single}. 
% These assumptions serve to restrict the solution spaces and enhance the recovery of reflection-free results. However, the performance of these methods is greatly compromised when these assumptions often do not hold, particularly in complex real-world reflection scenes. 

Recently, deep learning techniques have emerged as a promising direction, yielding substantial advancements in SIRR. Nevertheless, several bottlenecks still make existing learning-based methods struggle with real-world reflection scenes. One prominent issue is the limitations and expenses inherent to the previous data collection pipelines, which leads to a scarcity of high-quality, large-scale real pairs for training SIRR models. It's widely acknowledged that sufficient training samples are foundational for learning-based approaches. Yet, the existing collection pipelines frequently produce pairs with misalignment or artifacts.
 % On the one hand, due to the limitations and cost of the existing collection pipeline, there lack of high-quality, large-scale real pairs samples for training of SIRR models. Generally, sufficient training datasets are one of the most essential components for learning-based methods. However, existing collection pipelines often result in the non-alignment or artifacts in their collected pair images. 
% For example, pioneer works~\cite{zhang2018single, wei2019single,li2020single} capture the reflection-free images by removing the glass, which definitely brings the spatial pixel shift due to the glass refraction. Lei~\cite{lei2020polarized, lei2022categorized} exploits the linear reflection formation in the raw space and obtains the transmission layer by subtraction operation. However, the corresponding transmission contents still contain slight reflection residuals. Moreover, according to the previous collection pipeline, 
For instance, pioneering studies ~\cite{zhang2018single,wei2019single,li2020single} acquire reflection-free images by manually removing the glass. However, these approaches inevitably introduce spatial pixel non-alignment due to the refraction caused by the glass. Lei \etal \cite{lei2020polarized, lei2022categorized} leverage the linear reflection formation in raw space to derive the transmission layer via a subtraction process. Yet, we observe that this method leaves minor reflection remnants in the corresponding transmission layer. Moreover, considering the procedures or data format requirements of previous pipelines,  it will cost tremendously expensive labor and time to scale up the size of the datasets.

Another challenge is to distinguish the reflection and transmission contents within the captured images. This is attributed to the fact that the contents of the reflection layers also originate from the natural scenes.
% On the other hand, there is no specific pattern form for reflection components, and they are also derived from natural scenes, similar to the transmission layers. Hence, it makes particularly challenging.
% it is also challenging for SIRR to distinguish between reflection and transmission contents given input images.  
% Many previous methods~\cite{shih2015reflection,wan2018region,dong2021location, li2023two} adopt the divide-and-conquer strategy, reflection perception and removal, where reflection-related cues act as useful guidance to remove reflection effects. Wan \etal~\cite{wan2018region} obtain the reflection-dominated regions via the gradient prior, which often requires the uniform depth of field in the input images and specific hyper-parameter selection. Dong \etal ~\cite{dong2021location}  attempt to implicitly learn the reflection confidence map based on the linear composition loss. However, the linear formulation model cannot fully simulate real-world reflection scenarios. 
To enhance reflection removal, many established methods~\cite{shih2015reflection,wan2018region,dong2021location, li2023two} utilize a divide-and-conquer strategy, reflection perception and removal. Within these frameworks, cues related to reflections serve as valuable guidance for mitigating reflection artifacts. Wan \etal~\cite{wan2018region} assumes that the gradients of reflections are generally small and obtain the reflection-dominated regions via the threshold algorithm. Indeed, such an approach is not suitable for scenarios with strong reflections. 
%often requires the uniform depth of field in the input images and specific hyper-parameter selection. 
Dong \etal ~\cite{dong2021location} utilize the linear composition loss to implicitly infer the reflection confidence maps. Yet, their linear model often falls short in describing the complex real-world reflections. Despite such location cues have been shown to be effective in mitigating reflection disturbances as demonstrated by several studies~\cite{wan2017benchmarking, dong2021location, wan2018region}, it is rarely investigated the explicit representation to locate the reflection regions without specific assumptions.
%Despite such location cues being demonstrated to be effective in suppressing reflection disturbances~\cite{wan2017benchmarking, dong2021location,wan2018region},  




% To address the aforementioned challenges, we first propose a new collection pipeline of paired samples under real-world scenes and construct a high-quality large-scale reflection training dataset. To be specific,  we notice that reflection disturbances often arise when light from the camera side traverses the reflective material surfaces, subsequently interfering with the capture of the transmission layer. Therefore, we acquire the transmission layer without removing glasses, in which we employ non-transmissive and non-reflective black materials to block the reflective illumination. Then, we remove the light-blocking material to obtain images affected by reflective interference. Simultaneously, we conduct the overall process as the video capture mode, allowing for the intentional occlusion or creation of reflections to introduce diversity in reflection distortions.

To address the challenges previously delineated, firstly, we develop an innovative collection pipeline designed to procure paired samples from real-world scenarios, leading to the construction of a comprehensive, high-quality reflection training dataset. Specifically, it has been observed that reflections typically emerge when light from the camera's side intersects reflective material surfaces, thereby disturbing the clarity of the transmission layer. 
%
Hence, our method captures the transmission layer without the removal of glasses, utilizing non-transmissive and non-reflective black cloth to block reflection lights. Following this, the light-blocking materials are removed, facilitating the capture of images with reflection distortions. It is noteworthy that the whole process is executed in video mode, allowing the capture of dynamically changing reflections from the camera's perspective to enrich the diversity of reflection distortions.  These dynamic reflections could be from moving objects within the scenes or could be manually added or altered to enhance the reflection diversity.

Secondly, we observe the fact that the reflection layer encompasses textures of many virtual objects, which are absent in the corresponding ground-truth images. Therefore, we devise the maximum reflection filter (MaxRF) to explicitly present the reflection locations from the reflection pairs. Hence, we propose a cascaded SIRR network with reflection location-aware guidance. 
%
To be specific, under the guidance of the spatial location representation obtained from the MaxRF, the reflection detection network is first employed to learn to distinguish the reflection regions. Subsequently, these reflection location cues are incorporated into the reflection removal network, guiding the reflection removal process. 
% the detected reflection locations could be cascaded onto the restoration network to guide the removal of reflections. 
Finally, experimental results also demonstrate the effectiveness and the superiority of our proposed method. Our proposed dataset also will facilitate future research for SIRR.
%
 Contributions could be summarized as:
\begin{itemize}
  \item We propose a new pipeline for collecting reflection pairs. Compared with existing pipelines, ours is more applicable to various reflection scenarios without data format assumption, and it also allows for lower-cost acquisition of reflection pairs.

  \item We provide a large-scale high-quality paired reflection dataset, Reflection Removal in the Wild (RRW). To the best knowledge, RRW is the largest paired real-world reflection dataset, consisting of xxx image pairs with high resolution under various real-world reflection scenes.

  \item We develop a cascaded network for SIRR, which involves the reflection perception and removal network, \ie, first estimating location with the proposed maximum reflection filter and then removing reflections with location guidance. Comprehensive experiments indicate the superiority of the proposed innovations. 
\end{itemize}








==> tabs/SIR_comparisons.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h]
\caption{Quantitative comparisons on the subsets of real reflection benchmark~\cite{wan2017benchmarking}. The best results are in \textbf{bold}.}
\centering
\label{tab:SIR_subsets}
\begin{tabular}{crcccccc}
\toprule
\multirow{2}{*}{Methods} & \multicolumn{1}{c}{\multirow{2}{*}{Venue}} & \multicolumn{2}{c}{$wild(55)$}                             & \multicolumn{2}{c}{$postcard(199)$}                         & \multicolumn{2}{c}{$solid(200)$}                            \\  \cmidrule(l{2pt}r{2pt}){3-4}   \cmidrule(l{2pt}r{2pt}){5-6}  \cmidrule(l{2pt}r{2pt}){7-8}
                         & \multicolumn{1}{c}{}                       & PSNR                      & SSIM                     & PSNR                      & SSIM                     & PSNR                      & SSIM                     \\ \hline
Input Image              & \multicolumn{1}{c}{-}                      & 25.97                     & 0.90                     & 20.94                     & 0.87                     & 23.68                     & 0.89                     \\ \hline
FRS ~\cite{yang2019fast}                      & CVPR 20219                                 & \multicolumn{1}{l}{23.95} & \multicolumn{1}{l}{0.87} & \multicolumn{1}{l}{20.92} & \multicolumn{1}{l}{0.86} & \multicolumn{1}{l}{23.04} & \multicolumn{1}{l}{0.87} \\
ICBLN~\cite{li2020single}                    & CVPR 2020                                  & 24.41                     & 0.89                     & 23.25                     & 0.88                     & 24.75                     & 0.89                     \\
YTMT~\cite{hu2021trash}                     & NerIPS 2021                                & 25.23                     & 0.89                     & 2.23                      & 0.88                     & 24.46                     & 0.90                     \\
LANet~\cite{dong2021location}                    & ICCV 2021                                  & 25.89                     & 0.90                     & 21.27                     & 0.89                     & 24.00                     & 0.90                     \\
PNACR~\cite{wang2023personalized}                    & ACM MM 2023                                & 25.69                     & 0.90                     & 23.11                     & 0.89                     & 24.73                     & 0.89                     \\
DSRNet~\cite{hu2023single}                   & ICCV 2023                                  & 24.36                     & 0.89                     & 23.96                     & \textbf{0.89}            & 26.01                     & 0.92                     \\
Ours                     & \multicolumn{1}{c}{-}                      & \textbf{26.48}            & \textbf{0.91}            & \textbf{24.05}            & \textbf{0.89}            & \textbf{26.62}            & \textbf{0.93}            \\ \bottomrule
\end{tabular}
\end{table}

